Local Density Estimation in High Dimensions

An important question that arises in the study of high dimensional vector representations learned from data is: given a set $\mathcal{D}$ of vectors and a query $q$, estimate the number of points within a specified distance threshold of $q$. We develop two estimators, LSH Count and Multi-Probe Count that use locality sensitive hashing to preprocess the data to accurately and efficiently estimate the answers to such questions via importance sampling. A key innovation is the ability to maintain a small number of hash tables via preprocessing data structures and algorithms that sample from multiple buckets in each hash table. We give bounds on the space requirements and sample complexity of our schemes, and demonstrate their effectiveness in experiments on a standard word embedding dataset.

==> practical_considerations.tex <==

\section{Practical Implementation Considerations}

Our narrative so far has centered around motivating our general technique, whose theoretical sample and table complexity bounds depends on some key parameters. In this section, we provide greater perspective to practitioners  on how to design and customize this technique from data characteristics and their own available resources.
 
When choosing $\mathcal{I}$, the set of hamming distances to sample from, the tradeoff is that including more hamming distances reduces inherent bias in the estimate (which translates to fewer tables), but uses a higher sample complexity, and vice-versa. Practitioners have a sense of where they lie on this storage-runtime tradeoff frontier and can optimize for their particular situation.

The theoretical sample complexity also depends on $|{A}_q|$, which is the ground truth to be estimated. There are two general approaches to overcoming this issue in a practical context. The first is using domain knowledge -- most datasets 

For situations where one does not want to rely on prior knowledge, we discuss various stopping rules originating in the statistical literature on sequential analysis, where the problem is to determine when to stop sampling, based on previously gathered samples, in situations where the variance is unknown. 
 
Even though the sample complexity theoretically relies on $|{A}_q|$, the true number of near neighbors, in practice, implementers also understand a reasonable range for this number. For example, in our GLOVE dataset, the number of near neighbors typically fell into 3 categories, ~100, ~500, ~1000. Figure 3 shows that using 1000 samples and 20 tables could accurately assign the queries to their correct regimes. It is useful for a practitioner to be aware of this dependence, but for practical purposes, they can easily tune their parameters to achieve good results.

